Two- and three- dimensional few-body systems in the universal regime

Macro properties of cold atomic gases are driven by few-body correlations, even if the gas has thousands of particles. Quantum systems composed of two and three particles with attractive zero\=/range pairwise interactions are considered for general masses and interaction strengths in two and three dimensions (2D and 3D). The Faddeev decomposition is used to derive the equations for the bound state, which is the starting point for the investigation of universal properties of few\=/body systems, i.e. those that all potentials with the same physics at low energy are able to describe in a model\=/independent form. In 2D, the number of bound states in a three\=/body system increases without bound as the mass of one particle becomes much lighter than the other two. The analytic form of an effective potential between the heavy particles explains the mass\=/dependence on the number of bound energy levels. An exact analytic expression for the large\=/momentum asymptotic behaviour of the spectator function in the Faddeev equation is presented. The spectator function and its asymptotic form define the two- and three\=/body contact parameters. The two\=/body parameter is found to be independent of the quantum state in some specific 2D systems. The 2D and 3D momentum distributions have a distinct sub\=/leading form whereas the 3D term depends on the mass of the particles. A model that interpolates between 2D and 3D is proposed and a sharp transition in the energy spectrum of three-body systems is found.

==> preamble.tex <==
%%%%%%%%%%my packages%%%%%%%%%%
\usepackage{epsfig}
%\usepackage{cases}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{xcolor}

%\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{amssymb,bm}
\usepackage{amsmath}
\usepackage{color}
%\usepackage{bibunits}
\usepackage{graphicx}
\usepackage{todonotes}

\usepackage[latin1]{inputenc}
\usepackage{verbatim}

\usepackage{tikz}
%\usepackage{pgfmath}
\usetikzlibrary{calc}
\usepgflibrary{arrows}
\usepackage{bm}
\usepackage{hyperref}
\usepackage{cite}
\usepackage{multicol}

\usepackage{soul} % Til Daleifs forside
%\usepackage{siunitx}
%\usepackage[version=3]{mhchem}

%\usepackage{layouts} %bruges kun til at få side størrelse med printinunitsof
\setpagecc{\paperheight}{\paperwidth}{*}

\setlrmarginsandblock{*}{3cm}{0.75} % højre og venstre
\setulmarginsandblock{2.5cm}{*}{1}    % top og bund
\checkandfixthelayout[nearest]        % specifikt valg af højde algoritme

%\usepackage{lipsum}
%\usepackage{hyperref}
%note that hyperref seems to give problems with TeX-next-error in auctex just comment out to fix at error

%\usepackage{soul} % lege lege
%\sodef\an{}{0.2em}{.9em plus.6em}{1em plus.1em minus.1em}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


\usepackage{amstext}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{multirow}
\usepackage[section]{placeins}

\usepackage{epsfig}
\usepackage{epstopdf}
\usepackage{graphicx,color}  %
\usepackage{bm}  %


\usepackage{subfigure}
\usepackage{multirow}
\usepackage{color}
\usepackage{cases}

\usepackage[shortcuts]{extdash} % makes words like aaa-bbb be corrected spelled 

\usepackage{dsfont}

%\usepackage{cases}

%\setlength{\headheight}{27.12pt} %adjust the top of the page when chapter name is too long

\usepackage{MnSymbol} %use identity symbol

\allowdisplaybreaks[1] %allow equation to be split between pages


